Prime Match: A Privacy-Preserving Inventory Matching System

Inventory matching is a standard mechanism/auction for trading financial stocks by which buyers and sellers can be paired. In the financial world, banks often undertake the task of finding such matches between their clients. The related stocks can be traded without adversely impacting the market price for either client. If matches between clients are found, the bank can offer the trade at advantageous rates. If no match is found, the parties have to buy or sell the stock in the public market, which introduces additional costs. A problem with the process as it is presently conducted is that the involved parties must share their order to buy or sell a particular stock, along with the intended quantity (number of shares), to the bank. Clients worry that if this information were to leak somehow, then other market participants would become aware of their intentions and thus cause the price to move adversely against them before their transaction finalizes. We provide a solution, Prime Match, that enables clients to match their orders efficiently with reduced market impact while maintaining privacy. In the case where there are no matches, no information is revealed. Our main cryptographic innovation is a two-round secure linear comparison protocol for computing the minimum between two quantities without preprocessing and with malicious security, which can be of independent interest. We report benchmarks of our Prime Match system, which runs in production and is adopted by J.P. Morgan. The system is designed utilizing a star topology network, which provides clients with a centralized node (the bank) as an alternative to the idealized assumption of point-to-point connections, which would be impractical and undesired for the clients to implement in reality. Prime Match is the first secure multiparty computation solution running live in the traditional financial world.

==> mainFunctionality.tex <==
% !TEX root =  mainUSENIX.tex

\section{The Prime Match Main Functionalities}
\label{sec:prime-match}


We now describe our Prime Match inventory matching functionalities. We describe the bank-to-client functionality (Section~\ref{sec:func:bank-to-client}), the client-to-client functionality (Section~\ref{sec:func:client-to-client}), and the multi-client system (Section~\ref{sec:func:multiparty}). 

\subsection{Bank to Client Matching}
\label{sec:func:bank-to-client}
This variant is a two-party computation between a bank and a client. The bank tries to find matching orders between its own inventory and each client separately. As mentioned in the introduction, this essentially comes to replace the current procedure of axe-matching as being conducted today, with a privacy-preserving mechanism. Today the bank sends its inventory list to the client who then submits orders to the bank. 
%
Note, however, that if the bank runs twice with two different clients, and the bank does not hold some security {\tt X}, and two clients are interested in {\tt X} with opposite directions, then such a potential match will not be found.  %Client can see the axe list of the bank today (which contains information that relates to recent activities of other clients), 


\noindent
The functionality proceeds as follows. 
The client sends to the bank its axe list. This includes the list of securities it is interested in, and for each security whether it is interested in long (buy) or short (sell) exposures, and the quantity. The client sends its own list. The functionality finds whether the bank and the client are interested in the same securities with opposite sides, and in that case, it provides as output the 
matching orders and the quantity is the minimum between the two amounts. 

%dFor simplicity, we describe the functionality as there is only one particular security in the entire ``universe", and explain how to extend it to multiple securities below. %The system has two phases:



%{\bf Registration phase:} For each symbol, the client $P_i$ might wish to buy the particular security {\tt X} with either \emph{long} or \emph{short} exposure. The client sends to the functionality two integers, $L_i$ and $S_i$, corresponding to what amount it is interested in long exposure or short exposure, respectively. If the client is interested only in long exposure, then it sets $S_i=0$; if it is interested in short exposure, then it sets $L_i=0$. If it is not interested in both, it sends both as $0$. 




%Moreover, the client might have a range for each side; namely, it might interested in buying the stock, only if some minimal quantity is satisfied. As a result, the client sends to the server four different values: $((L_{\min}, L_{\max}), (S_{\min}, S_{\max}))$, corresponding to the two ranges. Of course, if the client is interested only in long exposure, then $(S_{\min},S_{\max})=(0,0)$; If interested in short exposure then it sets $(L_{\min}, L_{\max})$. %This is not enforced by the protocol, but it is irrational to have both sides non-zero as then the clients just pays extra fees. 


%The functionality maintains two lists, one for all short orders, and the other for the long orders, denoted as ${\cal L}$ and ${\cal S}$. The functionality inserts the orders to the lists in some random ordering, together with some meta information such as which client submitted this order (i.e., $P_i$). 

%The bank $P^*$, on its end, also sends its $L^*$, $S^*$ to the functionality. $L^*$ and $S^*$ are not inserted to ${\cal L}$ and ${\cal S}$. %commits to its list, i.e., values $L^*, S^*$ for the security ${\tt X}$. 
%\anti{So do we want to say that $L^*$, $S^*$ are also lists? since they are per symbol, or we should say earlier that we will focus in 1 symbol or make it clear that these $L^*$, $S^*$  are not added to the ${\cal L}$ and ${\cal S}$ lists}

% \medskip
% {\bf Matching phase:} The functionality iterates over the lists and matches each submitted value with the bank's values. This is essentially running minimum between the value $S_i$ obtained from ${\cal S}$ and $L^*$, where a secure, minimum sub-protocol is executed between the bank and the client that submitted the order. If a match was found, then both parties are notified with the matched amount; The parties are also notified if a match was not found. 

%If a match is found, it notifies both parties and the trade is executed. It then reduces from $L_{\sf bank}$, $S_{\sf bank}$


%and tries to first accommodate all clients as much as possible.  It compares $L^*$ with the list ${\cal S}$, while considering first only the ${S}_{\min}$ amounts of each client. If there is a match, then 

%and compares $S^*$ against the list ${\cal L}$. 

%\end{MyEnumerate}
% This process continues until the list ${\cal S}$ is empty, and is also repeated for the list ${\cal L}$ versus the input of the bank, $S^*$. 

% \medskip
% We generalize the above process to multiple securities in a natural manner -- the bank sends $L^*,S^*$ as lists of values and not just one, likewise each client. The number of possible symbols is around 1000-5000 and we can just process them all in parallel. Functionality~\ref{sec:func:bank-to-client} is described with only one security, for brevity. 
%
%For each possible security (or symbol), our functionality maintains \textit{first-in, first-out} queues, which respectively contain \textit{long} and \textit{short} orders (themselves encrypted integers) which are inserted in the queues in a random order. The number of possible symbols is around 1000-5000. When processing begins, the functionality repeatedly dequeues orders, performing a cryptographic minimum operation on each pair. To register an order of direction $d$ (valued either \textsc{Long} or \textsc{Short}) and volume $\mathsf{axe}$, a client encrypts $\mathsf{axe}$ as well as $0$ for the opposite direction, and submits both ciphertexts to the server (i.e., in an order which depends on $d$). This latter technique hides whether each order is long or short. If a client is not interested in a symbol then it inserts 0 for both sides $d$. We proceed as if the ``universe'' (the possible symbols) contained only one symbol; the process is repeated in parallel for multiple symbols.
%
%\paragraph{Bank-to-Client Matching.} In 
%Functionality~\ref{func:main1} we describe our main ideal functionality. For simplicity, we describe it for only one security, where generalizing it for all securities is done in a natural manner (in parallel).  

% The functionality is reactive; in particular, it proceeds in two stages. In the ``registration'' phase, $\mathcal{F}_{\text{main}}$ solicits integers $L$ and $S$ from the server and $({L}_\mathsf{min},{L}_\mathsf{max},{S}_\mathsf{min},{S}_\mathsf{max})$ from various parties $P_i$, enqueuing each integer it receives. $L$ refers to the Long encrypted orders and $S$ refers to the Short orders. Each client submits a minimum and a maximum number of shares they wish to trade either for the long $({L}_\mathsf{min},{L}_\mathsf{max})$ or for the short side $({S}_\mathsf{min},{S}_\mathsf{max})$. Clients submit zeros for the side they are not interested or zeros in both sides if they are not interested in the symbol. The bank submits a value for $S$ and a value for $L$, it does not submit a range of minimum and maximum number of shares. In the ``processing'' phase, $\mathcal{F}_{\text{main}}$ repeatedly compares the front-most integers of $\mathcal{L}_\mathsf{min}$ with 
%  $S$ to get the minimum value. If ${L}_\mathsf{min}$ is not zero and there is a match ($p=1$) the client sends the minimum quantity to the server. Once the server exhausts all the orders in ${L}_\mathsf{min}$ and ${S}_\mathsf{min}$, it applies the same process to ${L}_\mathsf{max}$ and ${S}_\mathsf{max}$. If there is no match, no party will not know if the minimum quantity of the other party was not satisfied or if the quantity was zero indicating that the party was not interested in that particular side and symbol.



\begin{mdframed}

\begin{functionality}[$\mathcal{F}_{\text{B2C}}$--Bank-to-client functionality]
\label{func:b2c}
The functionality is parameterized by the set of all possible securities to trade, a set $U$. 

\noindent
{\bf Input:} The bank $P^*$ inputs lists of orders $({\sf symb}_i^*, {\sf side}_i^*, {\sf amount}_i^*)$ where ${\sf symb}_i \subseteq U$ is the security, ${\sf side}_i^* \in \{{\sf buy}, {\tt sell}\}$ and ${\sf amount}_i^*$ is an integer. The client sends its list of the same format, $({\sf symb}_i^C, {\sf side}_i^C, {\sf amount}_i^C)$.


\noindent
{\bf Output:} Initialize a list of ${\sf Matches}$.
For each $i,j$ such that ${\sf symb}_i^* = {\sf symb}_j^C$ and ${\sf side}_i^* \neq {\sf side}_j^C$, add $({\sf symb}_i^*, {\sf side}_i^*, {\sf side}_j^C, \min\{{\sf amount}_i^*, {\sf amount}_j^C\})$ to $M$. Output $M$ to both parties. 
% \medskip
% \begin{MyEnumerate}
% \item Let $M = \min{L,S^*}$
% \end{MyEnumerate}

% Upon initialization, $\mathcal{F}_{\text{B2C}}$ initializes two lists, $\mathcal{L}$ and $\mathcal{S}$. 

% \medskip
% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Register}(P_i, L_i, S_i)$.} If $P_i$ has previously registered, then ignore the command. Otherwise, the values $L_i, S_i$ are inserted to (the same) random place in $\mathcal{L}$ and $\mathcal{S}$, respectively. Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 

% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Register}(P^*,L^*,S^*)$} Store the values $L^*$ and $S^*$. 

% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Process}()$}.
% \begin{MyEnumerate}
% \item Remove from ${\cal L}$ the top element, and let $L_i$ be that element with $P_i$ as the party sending that order to the bank. Send $P_i$ and $P^*$ the message ${\sf TryMatching}(P^*, P_i)$. 

% \item Let $M={\sf min}(L_i, S^*)$. If $M \neq 0$, then send ${\sf Match}(M)$ to $P^*$ and $P_i$, and set $S^* = S^*-M$. Otherwise, send ${\sf NoMatch}$ to both parties. 

% \item Repeat the above process (in parallel) for ${\cal S}$ and $L^*$. 

% \end{MyEnumerate}
\end{functionality}
\end{mdframed}

% \begin{mdframed}
% \begin{protocol}
% \noindent
% {\bf $\Pi_{\text{main}}.\textsf{Register}(P_i, L_i, S_i)$.} If $P_i$ sends to $P^*$ commitments of $L_i$, and $S_i$. $P^*$ inserts them to the lists ${\cal L}$ and ${\cal S}$ in a random order. 

% \noindent


% has previously registered, then ignore the command. Otherwise, the values $L_i, S_i$ are inserted to (the same) random place in $\mathcal{L}$ and $\mathcal{S}$, respectively. Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 
% \end{protocol}
% \end{mdframed}

% \begin{algorithmic}[1]
% \Procedure{$\mathcal{F}_{\text{main}}.\textsf{Register}(P_i, L_i, S_i)$}{}
% \State $\mathcal{L}_\mathsf{min}.\textsf{Enqueue}(\{ \mathsf{party}: P_i, \mathsf{axe}: L_\mathsf{min}\})$ where $P_i$ is the invoking $\mathsf{party}$ with $\mathsf{axe}$ minimum Long quantity $L_\mathsf{min}$.
% \State $\mathcal{L}_\mathsf{max}.\textsf{Enqueue}(\{ \mathsf{party}: P_i, \mathsf{axe}: L_\mathsf{max}\})$ where $P_i$ is the invoking $\mathsf{party}$ with $\mathsf{axe}$ maximum Long quantity $L_\mathsf{max}$.
% \State $\mathcal{S}_\mathsf{min}.\textsf{Enqueue}(\{ \mathsf{party}: P_i, \mathsf{axe}: S_\mathsf{min}\})$
% \State $\mathcal{S}_\mathsf{max}.\textsf{Enqueue}(\{ \mathsf{party}: P_i, \mathsf{axe}: S_\mathsf{max}\})$
% \EndProcedure
% \end{algorithmic}

% %\item 
% %When the registration phase ends, $\mathcal{F}_{\text{main}}$ executes the following function:
% \begin{algorithmic}[1]
% \Procedure{$\mathcal{F}_{\text{main}}.\textsf{Process}$}{\null}
% \While{\textbf{not} $\mathcal{L}_\mathsf{min}.\textsf{Empty}()$ and $S\neq 0$}
% \State $p := (\mathcal{L}_\mathsf{min}.\textsf{Front}().\textsf{axe}\leq S)$
% \State Send $p$ to $\mathcal{L}_\mathsf{min}.\textsf{Front}().\textsf{party}$
% \State If $p=1$ and $L_\mathsf{{min}}\neq 0$ send $v:=L_\mathsf{{min}}$ to $P^*$ 
% \State Set $S\mathrel{-}= v$
% \State $\mathcal{L}_\mathsf{min}.\textsf{Dequeue}()$
% \EndWhile
% \While{\textbf{not} $\mathcal{S}_\mathsf{min}.\textsf{Empty}()$ and $L\neq 0$}
% \State $p := (\mathcal{S}_\mathsf{min}.\textsf{Front}().\textsf{axe}\leq L)$
% \State Send $p$ to $\mathcal{S}_\mathsf{min}.\textsf{Front}().\textsf{party}$
% \State If $p=1$ and $S_\mathsf{{min}}\neq 0$ send $v:=S_\mathsf{{min}}$ to $P^*$ 
% \State Set $L\mathrel{-}= v$
% \State $\mathcal{S}_\mathsf{min}.\textsf{Dequeue}()$
% \EndWhile
% \State Repeat for $\mathcal{L}_\mathsf{max}$ and $\mathcal{S}_\mathsf{max}$
% \EndProcedure
% \end{algorithmic}
% %\end{MyItemize}
% \end{functionality}

From a business perspective, it is important to note that the input of the client serves as a ``commitment" - if a match is found then it is executed right away. Likewise the input of the bank.

The functionality resembles a set intersection. In set intersection, if some element is in the input set of some party but not in its output, it can conclude that it does not contain in the other set. Here, if a party does not find a particular symbol in its output although it did provide it as an input, then it is still uncertain whether the other party is not interested in that security, or whether it is interested but with the same side. 

We show how to implement the functionality in the presence of a malicious client or a semi-honest server in Appendix~\ref{sec:twoparty}.

\paragraph{Bank to multiple clients.}
In the actual system, the bank has to serve multiple clients. This is implemented by a simple (sequential) composition of the functionality. Specifically, the functionality is now reactive where clients first register that they are interested to participate. The bank then runs Functionality~\ref{func:b2c} with the clients -- either according to the basis of first-come-first-served, or some random ordering. We omit the details and exact formalism as they are quite natural given a semi-honest bank.  


\paragraph{Range functionalities.}
In Appendix~\ref{sec:range}, we show a variant of the protocol where each party inputs a \emph{range} in which it is interested and not just one single value. I.e., if a matched order does not satisfy some minimal value, it will not be executed. Since the minimum value does not change throughout the execution, whenever the bank receives $0$ as a result of the execution it cannot decide whether the client is not interested in that particular symbol, or whether it is interested -- but the matched amount does not satisfy the minimum threshold. 



\subsection{Client to Client Matching}
\label{sec:func:client-to-client}
In this variant, the bank has no input and it tries to find potential matches between clients facilitating two clients that wish to compare their inventories. This is a three-party computation where the bank just facilitates the interaction. It is important to notice that the clients do not know each other, and do not know who they are being paired with. The bank selects the two clients and offers them to be paired. 

%For simplicity of exposition, we describe the functionality as there is only one particular security and not a list of securities. 
\begin{mdframed}

\begin{functionality}[$\mathcal{F}_{\text{C2C}}$--Client-to-client functionality]
\label{func:c2c}
The functionality is parameterized by the set of all possible securities to trade, a set $U$. This is a three-party functionality between two clients, $P_1$ and $P_2$, and the bank $P^*$. 

\noindent
{\bf Input:} The client $P_1$ inputs a list of orders $({\sf symb}_i^{1}, {\sf side}_i^{1}, {\sf amount}_i^{1})$. \replaced{The client $P_2$ inputs a list of orders $({\sf symb}_i^{2}, {\sf side}_i^{2}, {\sf amount}_i^{2})$,}{The client $P_2$ inputs a list of the same format,} and the bank has no input. 

\noindent
{\bf Output:} Initialize a list of ${\sf Matches}$.
For each $i,j$ such that ${\sf symb}_i^{1} = {\sf symb}_j^{2}$ and ${\sf side}_i^{1} \neq {\sf side}_j^{2}$, add $({\sf symb}_i^{1}, {\sf side}_i^{1}, {\sf side}_j^{2}, \min\{{\sf amount}_i^{1}, {\sf amount}_j^{2}\})$ to $M$. Output $M$ to all three parties. 

% {\bf Input:} Client $P_i$ and $P_j$ inputs quantities $(L_i,S_i)$ and $(L_j,S_j)$.\\
% %Upon initialization, $\mathcal{F}_{\text{C2C}}$ initializes two lists, $\mathcal{L}$ and $\mathcal{S}$. 

% {\bf Output:} 
% \medskip
% \noindent
% {\bf $\mathcal{F}_{\text{C2C}}.\textsf{Register}(P_i, L_i, S_i)$.} If $P_i$ has previously registered, then ignore the command. Otherwise, the values $L_i, S_i$ are inserted to (the same) random place in $\mathcal{L}$ and $\mathcal{S}$, respectively. Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 

% \noindent
% {\bf $\mathcal{F}_{\text{C2C}}.\textsf{Process}()$}.
% \begin{MyEnumerate}
% \item Remove from ${\cal L}$ the top element, and let $L_i$ be that element with $P_i$ as the party sending that order to the bank. Remove from ${\cal S}$ the first element for a party $P_j$ for which $P_j\neq P_i$, and let $S_j$ be that element with $P_j$ as the party sending that order to the bank. Send $P_i,P_j$ and $P^*$ the message ${\sf TryMatching}(P_i, P_j)$. 

% \item Let $M={\sf min}(L_i, S_j)$. If $M \neq 0$ then
% \begin{enumerate}
%     \item Send ${\sf Match}(M)$ to $P_i$ and $P_j$.
%     \item Set $S_j = S_j-M$ and $L_i = L_i-M$.
%     \item For the case where $S_j\neq 0$ or $L_j\neq 0$ add orders back to the lists ${\cal S}$ and ${\cal L}$, respectively.
% \end{enumerate}
% Otherwise, send ${\sf NoMatch}$ to both parties. 

% \anti{Check that I am adding the orders back to the list}\gnote{where do you add them? is it really always random order?}

% \item Remove from ${\cal L}$ and ${\cal S}$ their top elements, let $L_i$, $S_j$ be the two top elements, and $P_i$ and $P_j$ the two contributing parties, respectively. 

% , and let $L_i$ be that element with $P_i$ as the parties sending that order to the bank. Send $P_i$ and $P^*$ the message ${\sf TryMatching}(P^*, P_i)$. 

% \item Let $M={\sf min}(L_i, S^*)$. If $M \neq 0$, then send ${\sf Match}(M)$ to $P^*$ and $P_i$, and set $S^* = S^*-M$. Otherwise, send ${\sf NoMatch}$ to both parties. 

% \item Repeat the above process (in parallel) for ${\cal S}$ and $L^*$. 

%\end{MyEnumerate}
\end{functionality}
\end{mdframed}
In the next section, we show how to implement this functionality in the presence of a malicious client or a malicious server, assuming that the two clients can communicate directly, or have a public-key infrastructure. When the two clients can communicate only through the server and there is no public-key infrastructure (PKI) or any other setup, there is no authentication and the server can impersonate the other client. We therefore cannot hope to achieve malicious security. We achieve security in the presence of a semi-honest server. See a discussion in the next subsection. 

\subsection{The Multi-Client System}
\label{sec:func:multiparty}
We now proceed to the multiparty auction. Here we have parties that register with their intended lists, and the bank facilitates the orders by pairing the clients according to some random order. 
The functionality is now reactive; The parties first register, in which they announce that they are willing to participate in the next auction, and they also commit to their orders. In the second phase, the bank selects pairs of clients in a random order to perform client-to-client matching. Looking ahead, typically there are around 10 clients that participate in a given auction. 
%\anti{should we mrntion here how many clients sre there for this use case? or where is the appropriate place?}

For simplicity of exposition and to ease readability, we write the functionality as the universe is just a single symbol. Moreover, instead of sending the side explicitly, the client sends two integers $L$ and $S$, representing its interest in long (buy) or short (sell) exposure, respectively. Rationally, each party would put one of the integers as $0$ (as otherwise, it would just pay extra fees to the bank). Generalizing the functionality to deal with many symbols is performed in a natural manner, where the number of total symbols is 1000-5000 in practice. The main functionality can process all the different symbols in parallel. 

\begin{mdframed}
\begin{functionality}[$\fmult$ -- Multi-client matching]
\label{func:multi}
This is an $n+1$ party functionality between $n$ clients $P_1,\ldots,P_n$ and a bank $P^*$. 

%{\bf Input:} Client $P_i$ inputs quantities $L_i$ and $S_i$.\\
Upon initialization, $\fmult$ initializes a list $\cal P=\emptyset$ and two vectors $\mathcal{L}$ and $\mathcal{S}$ of size $n$, where $n$ bounds the total number of possible clients. 

\medskip
\noindent
{\bf $\fmult.\textsf{Register}(P_i, L_i, S_i)$.} 
Store $\mathcal{L}[i] = L_i$ and $\mathcal{S}[i] = S_i$ and add $i$ to $\cal P$. 
Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 

\noindent
{\bf $\fmult.\textsf{Process}()$}.
\begin{enumerate}[nosep]
\item Choose a random ordering $O$ over all pairs of $\cal P$. 
\item For the next pair $(i,j) \in O$ try to match between $P_i$ and $P_j$ (we can assume wlog that always $i \leq j$): 
\begin{enumerate}[leftmargin=*]
\item Compute $M_0 = {\sf min}({\cal L}[i], {\cal S}[j])$, $b_0^0 = ({\cal L}[i] \leq {\cal S}[j])$, $b_1^0 = ({\cal S}[i] \leq {\cal L}[j])$. 
\item Compute $M_1 = {\sf min}({\cal S}[i], {\cal L}[j])$, $b_0^1 = ({\cal S}[i] \leq {\cal L}[j])$ and $b_1^1 = ({\cal S}[i] \leq {\cal L}[j])$. 
\item Send $(i,j,M_0,M_1, b_i^0,b_i^1)$ to $P_i$, and $(i,j,M_0,M_1)$ with $(b_0^0,b_1^0,b_0^1,b_1^1)$ to $P^*$.%\anti{wait in the protocol the Ms are revealed after the bs} 
\item Update ${\cal L}[i] = {\cal L}[i]-M_0$ and ${\cal S}[j] = {\cal S}[j]-M_0$. 
\item Update ${\cal S}[i] = {\cal S}[i]-M_1$ and ${\cal L}[j] = {\cal L}[j]-M_1$.
\end{enumerate}
\end{enumerate}




%
%\item Remove from ${\cal L}$ the top element, and let $L_i$ be that element with $P_i$ as the party sending that order to the bank. Remove from ${\cal S}$ the first element for a party $P_j$ for which $P_j\neq P_i$, and let $S_j$ be that element with $P_j$ as the party sending that order to the bank. Send $P_i,P_j$ and $P^*$ the message ${\sf TryMatching}(P_i, P_j)$. 
%
%\item Let $M={\sf min}(L_i, S_j)$. If $M \neq 0$ then
%\begin{enumerate}
%    \item Send ${\sf Match}(M)$ to $P_i$ and $P_j$.
%    \item Set $S_j = S_j-M$ and $L_i = L_i-M$.
%    \item For the case where $S_j\neq 0$ or $L_j\neq 0$ add orders back to the top if the lists ${\cal S}$ and ${\cal L}$, respectively.
%\end{enumerate}
%Otherwise, send ${\sf NoMatch}$ to both parties. 
%
%%\anti{Check that I am adding the orders back to the list}\gnote{where do you add them? is it really always random order?}
%
%% \item Remove from ${\cal L}$ and ${\cal S}$ their top elements, let $L_i$, $S_j$ be the two top elements, and $P_i$ and $P_j$ the two contributing parties, respectively. 
%
%% , and let $L_i$ be that element with $P_i$ as the parties sending that order to the bank. Send $P_i$ and $P^*$ the message ${\sf TryMatching}(P^*, P_i)$. 
%
%% \item Let $M={\sf min}(L_i, S^*)$. If $M \neq 0$, then send ${\sf Match}(M)$ to $P^*$ and $P_i$, and set $S^* = S^*-M$. Otherwise, send ${\sf NoMatch}$ to both parties. 
%
%% \item Repeat the above process (in parallel) for ${\cal S}$ and $L^*$. 
%\end{MyEnumerate}
%
%\end{MyEnumerate}
\end{functionality}
\end{mdframed}

\paragraph{On malicious server.}
Our final protocol (see Appendix~\ref{sec:mainprotocol}) for $\fmult$ is secure in the presence of a semi-honest $P^*$ (and a malicious client). Inherently, clients communicate through a star network where the bank facilitates the communication. Moreover, we assume no PKI, clients do not know how many clients are registered in the system, and how many clients are participating in the current auction. %\anti{isnt registered and participating in the current auction the same thing?}\gnote{not really. one is "the bank offered me to participate" and the other is "I am actively participating in the current auction"}
This can be viewed as ``secure computation without authentication", in which case the server can always ``split" the communication and disconnect several parties from others (see~\cite{BarakCLPR11} for a formal treatment). 


%Since we inherently cannot guarantee security against a malicious server, and the bank has to execute the matching orders immediately, 
We prove security in the presence of a semi-honest server. In fact, our protocol achieves a stronger notion of a guarantee than just semi-honest, as in particular, it runs the underlying comparison protocol (a single invocation of a client-to-client matching) which is secure against a malicious server.  

Another relaxation that we make is that the ordering of pairs is random, and we do not have a mechanism to enforce it. %\anti{should we say that the bank will follow the order for reputation reasons?} 
%This can be enforced by running some coin tossing between the parties and having some bulletin board in which they can view that the matching that is being executed is between the next pair. \anti{if we have a bulletin board then the parties will know the number of the other parties etc. }
%
%
%
 Note also that the functionality leaks some information to the server; in particular, after finding a match, the bank executes it immediately. The bank can infer information about whether two values equal to $0$, and therefore whether a client is not interested in a particular symbol. In contrast, each client just learns whether its value is smaller or equal to the value of the other party, and therefore when it inputs $0$ it can never infer whether the other party is interested in that symbol or not. 



%the clients have to trust the server that it indeed tries to pair them with all participants, we take the following simplifying assumptions on the behaviour of the server (the bank): 
%\gnote{to continue - what are the assumptions? if you can continue it will be great}\anti{wait do we want to say here that we are assuming that the server tosses a coin to choose the order of the clients and to the best of his interest due to reputation risk he follows the order? Do we want to fit here also the fact that the server only inputs 1 non zero L and S to avoid leaking client's interests per symbol (i.e. hiding the symbol). I  guess there is also the leakage of learning some info if a client is tried to be matched with lets say 3 clients and we only get a match in the 4th try with a 4th client, perhaps it can tell what the previous 3 orders did not have as quantities, I think we wrote something about this leakage at the rebuttal)}





%The protocol for implementing this functionality is given in Protocol~\ref{prot:main} in Appendix~\ref{sec:mainprotocol}. It is just based on a secure protocol for computing the minimum as a building block, a protocol of the latter is given in Section~\ref{sec:minimum}. 
%
%
%\anti{I guess i should also update the functionalities with the minimum quantities in the appendix to follow this new format of the functionalities and we somehow need to cite those functionaliotes from this section}




==> range_functionalities.tex <==


\section{Range Functionalities}
\label{sec:range}

\subsection{Range Bank-to-Client Functionality}

In this section we consider a modification to Functionality~\ref{func:b2c}. in which the client submits a minimum and a maximum amount per stock instead of a single amount. 

\begin{mdframed}

\begin{functionality}[$\mathcal{F}_{\text{B2C}}$--Bank-to-client functionality]
\label{func:b2cv2}
The functionality is parameterized by the set of all possible securities to trade, a set $U$. 

\noindent
{\bf Input:} The bank $P^*$ inputs lists of orders $({\sf symb}_i^*, {\sf side}_i^*, {\sf amount}_i^*)$ where ${\sf symb}_i \subseteq U$ is the security, ${\sf side}_i^* \in \{{\sf long}, {\tt short}\}$ and ${\sf amount}_i^*$ is an integer. The client sends its list of the same format but with a minimum and a maximum amount, $({\sf symb}_i^C, {\sf side}_i^C, {\sf MinAmount}_i^C,{\sf MaxAmount}_i^C)$.


\noindent
{\bf Output:} Initialize a list of ${\sf Matches}$ $M$.
For each $i,j$ such that ${\sf symb}_i^* = {\sf symb}_j^C$ and ${\sf side}_i^* \neq {\sf side}_j^C$, %add $({\sf symb}_i^*, {\sf side}_i^*, {\sf side}_j^C, \min\{{\sf amount}_i^*, {\sf MinAmount}_j^C\})$ to $M$. 
then if
${\sf amount}_i^* > {\sf MinAmount}_j^C$, then add  $({\sf symb}_i^*, {\sf side}_i^*, {\sf side}_j^C, \min\{{\sf amount}_i^*, {\sf MaxAmount}_j^C\})$ to $M$. Output $M$ to both parties. 
% \medskip
% \begin{MyEnumerate}
% \item Let $M = \min{L,S^*}$
% \end{MyEnumerate}

% Upon initialization, $\mathcal{F}_{\text{B2C}}$ initializes two lists, $\mathcal{L}$ and $\mathcal{S}$. 

% \medskip
% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Register}(P_i, L_i, S_i)$.} If $P_i$ has previously registered, then ignore the command. Otherwise, the values $L_i, S_i$ are inserted to (the same) random place in $\mathcal{L}$ and $\mathcal{S}$, respectively. Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 

% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Register}(P^*,L^*,S^*)$} Store the values $L^*$ and $S^*$. 

% \noindent
% {\bf $\mathcal{F}_{\text{B2C}}.\textsf{Process}()$}.
% \begin{MyEnumerate}
% \item Remove from ${\cal L}$ the top element, and let $L_i$ be that element with $P_i$ as the party sending that order to the bank. Send $P_i$ and $P^*$ the message ${\sf TryMatching}(P^*, P_i)$. 

% \item Let $M={\sf min}(L_i, S^*)$. If $M \neq 0$, then send ${\sf Match}(M)$ to $P^*$ and $P_i$, and set $S^* = S^*-M$. Otherwise, send ${\sf NoMatch}$ to both parties. 

% \item Repeat the above process (in parallel) for ${\cal S}$ and $L^*$. 

% \end{MyEnumerate}
\end{functionality}
\end{mdframed}





\gnote{write something about the protocol?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Range Client-to-Client Functionality}


In this section, we show how to modify the original functionality to accommodate client to client matching satisfying the requirement that the matched quantity should be between the minimum and the maximum quantities of each client. In particular, each client will submit both a maximum amount and a minimum amount. If the ranges of the orders for the two clients  $[L_\mathsf{min}, L_\mathsf{max}]$  and $[S_\mathsf{min}, S_\mathsf{max}]$\anti{this text is updated  jutt the notation for Lmax and Lmix, Smax and Smin is not updated  to be consistent with the boxed of the functionalities} intersect then we know that both client’s range requirements will be met, and the trading volume will be  in this intersection. To examine the intersection, we perform secure comparison over these values, so that we can learn whether they intersect without learning any of the individual values. 









As an example, suppose the range of the buy order is $[50,100]$ and the range of the sell order is $[25,75]$. Computing the matches proceeds as follows: first, compare the minimum buy order with the maximum sell order $(L_\mathsf{min} \leq S_\mathsf{max})$ and the minimum sell order with the maximum buy order $(S_\mathsf{min} \leq L_\mathsf{max})$. If both comparison bits are 1 then the ranges intersect and we execute and find the minimum between the buy quantity and the maximum sell quantity. This will result in a trading volume of 50. Since this fully exhausts the buyer’s minimum orders, the quantity is fully revealed (but the maximum buy order cannot be revealed). 

Next, we must make sure that the seller meets their minimum selling requirement. To do so, we must first update the orders based on the results of the previous round. Since the previous matched transaction is public, we can subtract the matched quantity of the previous round from the clients respective order(s) including the maximum buy quantity. After the orders are updated, we check again
if $(L_\mathsf{min} \leq S_\mathsf{max})$ and  $(S_\mathsf{min} \leq L_\mathsf{max})$. If it is both predicates are true then we execute the minimum sell order. This will guarantee that all minimum order requirements are satisfied. 

Once all minimum order requirements are satisfied, we can once again update the orders by subtracting the quantities of the new public transaction. At this point, all order ranges are of the form $[0,k]$, since all minimum order requirements have already been satisfied. We execute the protocol one more time on these remaining maximum orders and this completes our extended protocol. Note that the total trading volume ends up being not just any value in the original range intersection, but actually the maximum value in that intersection. So in the example, we would end up matching 75 units.

Note that if the comparison bits are not equal to 1 then the ranges do not intersect and there is no match.




\begin{mdframed}
\begin{functionality}[$\mathcal{F}_{\text{C2C}}$--Client-to-client functionality]
\label{func:c2cv2}
The functionality is parameterized by the set of all possible securities to trade, a set $U$. This is a three party functionality between two clients, $P_1$ and $P_2$, and the bank $P^*$. 

\noindent
{\bf Input:} The client $P_1$ inputs a list of orders $({\sf symb}_i^{1}, {\sf side}_i^{1}, {\sf MinAmount}_i^{1},{\sf MaxAmount}_i^{1})$. The client $P_2$ inputs a list of the same format, and the bank has no input. 

\noindent
{\bf Output:} Initialize a list of ${\sf Matches}$.
For each $i,j$ such that ${\sf symb}_i^{1} = {\sf symb}_j^{2}$ and ${\sf side}_i^{1} \neq {\sf side}_j^{2}$:
\begin{itemize}
    \item If $({\sf MinAmount}_i^{1}\leq{\sf MaxAmount}_j^{2})$ and $({\sf MinAmount}_j^{2}\leq{\sf MaxAmount}_i^{1})$ add $({\sf symb}_i^{1}, {\sf side}_i^{1}, {\sf side}_j^{2},m_1:= {\sf MinAmount}_i^{1})$ to $M$ else break;\anti{not clear if this break is enough, I want to basically mean that in this case there is no match and we do not move to the second item below}
    \item If $({\sf MinAmount}_i^{1}-m_1\leq{\sf MaxAmount}_j^{2}-m_1)$ and $({\sf MinAmount}_j^{2}\leq{\sf MaxAmount}_i^{1}-m_1)$ add $({\sf symb}_i^1, {\sf side}_i^1, {\sf side}_j^2, m_2={\sf MinAmount}_j^2)$ to $M$ else break;\anti{Gilad did you ask here if this can be done without subtraction?I just thought about it and i dont think so }
    
    
    %and $({\sf symb}_i^{1}, {\sf side}_i^{1}, {\sf side}_j^{2}, m_2:={\sf MinAmount}_j^{2})$ else break; 
    \item Add $({\sf symb}_i^1, {\sf side}_i^1, {\sf side}_j^2, \min\{{\sf MaxAmount}_i^1- m_1-m_2 , {\sf MaxAmount}_j^2-m_1-m_2\})$ to $M$.
    

    
\end{itemize}

% {\bf Input:} Client $P_i$ and $P_j$ inputs quantities $(L_i,S_i)$ and $(L_j,S_j)$.\\
% %Upon initialization, $\mathcal{F}_{\text{C2C}}$ initializes two lists, $\mathcal{L}$ and $\mathcal{S}$. 

% {\bf Output:} 
% \medskip
% \noindent
% {\bf $\mathcal{F}_{\text{C2C}}.\textsf{Register}(P_i, L_i, S_i)$.} If $P_i$ has previously registered, then ignore the command. Otherwise, the values $L_i, S_i$ are inserted to (the same) random place in $\mathcal{L}$ and $\mathcal{S}$, respectively. Send to the bank $P^*$ the message ${\sf registered}(P_i)$. 

% \noindent
% {\bf $\mathcal{F}_{\text{C2C}}.\textsf{Process}()$}.
% \begin{MyEnumerate}
% \item Remove from ${\cal L}$ the top element, and let $L_i$ be that element with $P_i$ as the party sending that order to the bank. Remove from ${\cal S}$ the first element for a party $P_j$ for which $P_j\neq P_i$, and let $S_j$ be that element with $P_j$ as the party sending that order to the bank. Send $P_i,P_j$ and $P^*$ the message ${\sf TryMatching}(P_i, P_j)$. 

% \item Let $M={\sf min}(L_i, S_j)$. If $M \neq 0$ then
% \begin{enumerate}
%     \item Send ${\sf Match}(M)$ to $P_i$ and $P_j$.
%     \item Set $S_j = S_j-M$ and $L_i = L_i-M$.
%     \item For the case where $S_j\neq 0$ or $L_j\neq 0$ add orders back to the lists ${\cal S}$ and ${\cal L}$, respectively.
% \end{enumerate}
% Otherwise, send ${\sf NoMatch}$ to both parties. 

% \anti{Check that I am adding the orders back to the list}\gnote{where do you add them? is it really always random order?}

% \item Remove from ${\cal L}$ and ${\cal S}$ their top elements, let $L_i$, $S_j$ be the two top elements, and $P_i$ and $P_j$ the two contributing parties, respectively. 

% , and let $L_i$ be that element with $P_i$ as the parties sending that order to the bank. Send $P_i$ and $P^*$ the message ${\sf TryMatching}(P^*, P_i)$. 

% \item Let $M={\sf min}(L_i, S^*)$. If $M \neq 0$, then send ${\sf Match}(M)$ to $P^*$ and $P_i$, and set $S^* = S^*-M$. Otherwise, send ${\sf NoMatch}$ to both parties. 

% \item Repeat the above process (in parallel) for ${\cal S}$ and $L^*$. 

%\end{MyEnumerate}
\end{functionality}
\end{mdframed}


\anti{if you agree with the above format then i will write the multiclient one, or do we need to specify the details of the multiclient? Btw I think here we need an intermediate functionality in which the bank first goes over all the minimum quantities of the clients and then checks their maximum quantities (recall that this is what is really running in production right now) until the banks inventory is excused}


%%%%%%%%%%%%%%%%%%%%%%%%%%

The current system is set to accept a minimum and a maximum quantity to be matched from the clients. As a first step, the bank runs Functionality~\ref{func:b2c} on every client one by one only on their minimum quantity until the bank exhausts its inventory. For the case where the bank did not exhaust its inventory after processing all the clients, it runs again Functionality~\ref{func:b2c} on every client one by one on their maximum quantity. This process is presented in Functionality~\ref{func:b2cv2}. The requirement on the minimum and maximum quantity is imposed by the business for this use case as a greedy approach in an effort to satisfy more clients with the bank's inventory. This is not a necessary requirement but the bank views it as an additional feature to satisfy more clients. This greedy approach is not ideal since, for instance, the minimum quantity of the first client can exshaust the full inventory of the bank. We leave it as an open problem to devise a secure optimization algorithm for better allocations across all clients. %The current method performs well in practice. In particular, there is enough daily inventory to process the minimum quantities of a large number of clients (if not all).  



%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{mdframed}

\begin{functionality}[$\mathcal{F}_{\text{B2C}}$--Bank-to-multiclient functionality]\anti{change the name}
\label{func:b2cv2}
The functionality is parameterized by the set of all possible securities to trade, a set $U$. 

\noindent
{\bf Input:} The bank $P^*$ inputs lists of orders $({\sf symb}_i^*, {\sf side}_i^*, {\sf amount}_i^*)$ where ${\sf symb}_i \subseteq U$ is the security, ${\sf side}_i^* \in \{{\sf long}, {\tt short}\}$ and ${\sf amount}_i^*$ is an integer. A client $P_i$ sends its list of the same format but with a minimum and a maximum amount, $({\sf symb}_i^C, {\sf side}_i^C, {\sf MinAmount}_i^C,{\sf MaxAmount}_i^C)$.


\noindent
{\bf Output:} Initialize a list of ${\sf Matches}$ $M$. While ${\sf amount}_i^{*}\neq 0$:
\begin{itemize}
    \item For each $j$ (chosen in a random order) such that ${\sf symb}_i^{*} = {\sf symb}_j^{C}$ and ${\sf side}_i^{*} \neq {\sf side}_j^{C}$, add $({\sf symb}_i^{*}, {\sf side}_i^{*}, {\sf side}_j^{C}, \min\{{\sf amount}_i^{*}, {\sf MinAmount}_j^{C}\})$ to $M$ and update ${\sf amount}_i^{*}$. 
 

    \item For each $j$ (chosen  in a random order) present in $M$ such that ${\sf symb}_i^{*} = {\sf symb}_j^{C}$ and ${\sf side}_i^{*} \neq {\sf side}_j^{C}$, add $({\sf symb}_i^{*}, {\sf side}_i^{*}, {\sf side}_j^{C}, \min\{{\sf amount}_i^{*}, {\sf MaxAmount}_j^{C}-{\sf MinAmount}_j^{C}\})$ to $M$ and update ${\sf amount}_i^{*}$. \anti{in this last one we can actually have it $\min\{{\sf amount}_i^{*}, {\sf MaxAmount}_j^{C}\}$if the clients inputs as max value the excess value in the registration phase}
\end{itemize}



\end{functionality}
\end{mdframed}

